EEG-GCNN: Augmenting Electroencephalogram-based Neurological Disease Diagnosis using a Domain-guided Graph Convolutional Neural Network

This paper presents a novel graph convolutional neural network (GCNN)-based approach for improving the diagnosis of neurological diseases using scalp-electroencephalograms (EEGs). Although EEG is one of the main tests used for neurological-disease diagnosis, the sensitivity of EEG-based expert visual diagnosis remains at $\sim$50\%. This indicates a clear need for advanced methodology to reduce the false negative rate in detecting abnormal scalp-EEGs. In that context, we focus on the problem of distinguishing the abnormal scalp EEGs of patients with neurological diseases, which were originally classified as 'normal' by experts, from the scalp EEGs of healthy individuals. The contributions of this paper are three-fold: 1) we present EEG-GCNN, a novel GCNN model for EEG data that captures both the spatial and functional connectivity between the scalp electrodes, 2) using EEG-GCNN, we perform the first large-scale evaluation of the aforementioned hypothesis, and 3) using two large scalp-EEG databases, we demonstrate that EEG-GCNN significantly outperforms the human baseline and classical machine learning (ML) baselines, with an AUC of 0.90.

==> further_analysis.tex <==
\section{Posthoc Analysis}

\noindent \textbf{Statistical comparisons:} 
 Furthermore, we suspected that older healthy subjects (taken from LEMON dataset) might show higher disease probability than younger subjects \textcolor{red}{citation needed?}. We applied a one-way ANOVA test and found a non-significant p-value ($p>0.05$), suggesting that different age groups do not show significantly different disease risk under both shallow and deep GNN models.

% - Our results indicate that graph neural network based models outperform the traditional machine learning and deep learning baselines for this task. Interestingly, within the class of GNNs, the shallow GNN model (2 Graph Conv layers) outperforms the deep GNN model (5 Graph Conv layers). The depth limitation of GNNs has been previously acknowledged [??] and multiple previous GNN-based studies report downward trends in performance as the number of graph convolution layers increase, even just beyond 2-4 layers. [cite https://arxiv.org/pdf/1909.12223.pdf]


% - The 128-dimensional graph embeddings learned by the shallow GNNs show promising separability between the two classes in 2D/3D space (see Figure for tSNE visualization). A deeper inspection of embedding clusters and the variability of subjects' predictions across the ten folds is left as future work.


==> implementation.tex <==
\section{Implementation}

The shallow variant of EEG-GCNN comprises only of 2 Graph Convolution layers (output emdedding dimensions: 64, 128) and a Global Mean Pooling layer. Notably, the shallow EEG-GCNN has no hidden Linear layers. In contrast, the deep variant of EEG-GCNN, is composed of 5 Graph Convolution layers (output emdedding dimensions: 16, 16, 32, 64, 128), a Global Mean Pooling layer, and 2 hidden Linear layers (hidden dimensions: 30, 20). The baseline Fully-connected Neural Network comprises 2 hidden Linear Layers (hidden dimensions: 64, 32). The Random Forest baseline is made up of 100 weak decision tree learners, with 4 features considered for node splitting, and a maximum tree depth of 15. The bagging fraction was taken to be 20\% of the training set, and the complexity parameter for tree pruning was set to 0.015. The hyperparameter tuning process for these models is described in \textcolor{red}{section \ref{sec:}.} Model implementations were done using the Scikit-learn, PyTorch, and PyTorch Geometric libraries \cite{pedregosa2011scikit}, \cite{paszke2019pytorch}, \cite{fey2019fast}.

% HYPERPARAMS = {'ccp_alpha': 0.015, 'class_weight': 'balanced', 'criterion': 'gini', 'max_depth': 15, 'max_features': 4, 'max_samples': 0.2, 'min_samples_leaf': 15, 'min_samples_split': 2, 'n_estimators': 100}  


